Privacy Leakage in Discrete Time Updating Systems

A source generates time-stamped update packets that are sent to a server and then forwarded to a monitor. This occurs in the presence of an adversary that can infer information about the source by observing the output process of the server. The server wishes to release updates in a timely way to the monitor but also wishes to minimize the information leaked to the adversary. We analyze the trade-off between the age of information (AoI) and the maximal leakage for systems in which the source generates updates as a Bernoulli process. For a time slotted system in which sending an update requires one slot, we consider three server policies: (1) Memoryless with Bernoulli Thinning (MBT): arriving updates are queued with some probability and head-of-line update is released after a geometric holding time; (2) Deterministic Accumulate-and-Dump (DAD): the most recently generated update (if any) is released after a fixed time; (3) Random Accumulate-and-Dump (RAD): the most recently generated update (if any) is released after a geometric waiting time. We show that for the same maximal leakage rate, the DAD policy achieves lower age compared to the other two policies but is restricted to discrete age-leakage operating points.

==> DTQueueAgeFigure.tex <==

\subsection{Age at the Monitor for a Queueing Server}
When the server is a first-come first-served queue, an age sample path $A_m(t)$ at the monitor is depicted in Fig.~\ref{fig:DTqueue}. In the queue, $T_k$ denotes the system time of the $k$th update. The average age is still given by \eqnref{sum-age} with $A(n)=A_m(t)$ but now we decompose the area under the age process into areas $Q_k$ that equal the difference of the $Y_k+T_k$-step staircase area and the $T_k$-step staircase area. Thus,
\begin{align}
    Q_k&=\frac{(Y_k+T_k)(Y_k+T_k+1)}{2} -\frac{T_k(T_k+1)}{2}\nn
    &=Y_k^2/2 +T_kY_k +Y_k/2.
\end{align}
Employing the same steps as in \eqnref{queue-input-age}, we obtain the average age
\begin{align}
    \E{A_m(t)}
    &=\frac{\E{Q_k}}{\E{Y_k}}=\frac{\E{Y_k^2}+2\E{Y_kT_k}}{2\E{Y_k}}+\frac{1}{2}.
    \eqnlabel{queue-output-age}
\end{align}

\begin{figure}[t]%Queue fig
    \centering
\begin{tikzpicture}[scale=\linewidth/28cm]
\draw [<->] (0,10) node [above] {$A_m(n)$} -- (0,0) --  (23,0) node [right] {$n$};
\draw [thin]\xtic{1}\xtic{2}\xtic{3}\xtic{4}\xtic{5}\xtic{6}\xtic{7}
\xtic{8}\xtic{9}\xtic{10}\xtic{11}\xtic{12}\xtic{13}\xtic{14}\xtic{15}\xtic{16}\xtic{17}\xtic{18}\xtic{19}\xtic{20}\xtic{21}\xtic{22}; 
\draw [thin]\ytic{1}\ytic{2}\ytic{3}\ytic{4}\ytic{5}\ytic{6}\ytic{7}\ytic{8}\ytic{9};
\fill [pattern=north west lines, pattern color=blue] (3,0) 
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,-5)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0) --(3,0);
\fill [fill=lightgray] (8,0) 
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,-2)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0) --(8,0);
\draw [thick] 
(0,1) -- ++(1,0) -- 
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,-2) -- ++(1,0) -- % update #1
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,-4)-- ++(1,0) -- %update #2
++(0,-1)-- ++(1,0) -- %update #3
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,-4) -- ++(1,0) -- %update #3
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0);
\draw (2,0) node [below] {$n_1$};
\draw [->] (5,0) -- ++(0,-1) node [below] {$n'_1$};
\draw (7,0) node [below] {$n_2$}; 
\draw (9,0) node [below] {$n_3$};
\draw [->] (12,0) -- ++(0,-1) node [below] {$n'_2$};
\draw [->] (13,0) -- ++(0,-1) node [below] {$n'_3$};
\draw  [|<->|] (0,-3.5) to node [below] {$Y_1$} ++(3,0);
\draw  [|<->|] (3,-3.5) to node [below] {$T_1$} ++(2,0);
\draw  [|<->|] (3,-5.5) to node [below] {$Y_2$} ++(5,0);
\draw  [|<->|] (8,-5.5) to node [below] {$T_2$} ++(4,0);
\draw  [|<->|] (8,-3.5) to node [below] {$Y_3$} ++(2,0);
\draw  [|<->|] (10,-3.5) to node [below] {$T_3$} ++(3,0);
\draw[<-] (12.5,3.5) to [out=110,in=250] ++(1,4) node [above] {$Q_3$};
\draw[<-] (7.5,3.5) to [out=110,in=250] ++(1,4) node [above] {$Q_2$};
\end{tikzpicture}
\caption{The age process $A_m(n)$ at the monitor when updates from the source pass through a queue. %(The system is initialized with a fresh arrival prior to slot $0$.
}
\label{fig:DTqueue}
\end{figure}

==> Privacy Leakage/DTQueueAgeFigure.tex <==

\subsection{Age at the Monitor for a Queueing Server}
When the server is a first-come first-served queue, an age sample path $A_m(t)$ at the monitor is depicted in Fig.~\ref{fig:DTqueue}. In the queue, $T_k$ denotes the system time of the $k$th update. The average age is still given by \eqnref{sum-age} with $A(n)=A_m(t)$ but now we decompose the area under the age process into areas $Q_k$ that equal the difference of the $Y_k+T_k$-step staircase area and the $T_k$-step staircase area. Thus,
\begin{align}
    Q_k&=\frac{(Y_k+T_k)(Y_k+T_k+1)}{2} -\frac{T_k(T_k+1)}{2}\nn
    &=Y_k^2/2 +T_kY_k +Y_k/2.
\end{align}
Employing the same steps as in \eqnref{queue-input-age}, we obtain the average age
\begin{align}
    \E{A_m(t)}
    &=\frac{\E{Q_k}}{\E{Y_k}}=\frac{\E{Y_k^2}+2\E{Y_kT_k}}{2\E{Y_k}}+\frac{1}{2}.
    \eqnlabel{queue-output-age}
\end{align}

\begin{figure}[t]%Queue fig
    \centering
\begin{tikzpicture}[scale=\linewidth/28cm]
\draw [<->] (0,10) node [above] {$A_m(n)$} -- (0,0) --  (23,0) node [right] {$n$};
\draw [thin]\xtic{1}\xtic{2}\xtic{3}\xtic{4}\xtic{5}\xtic{6}\xtic{7}
\xtic{8}\xtic{9}\xtic{10}\xtic{11}\xtic{12}\xtic{13}\xtic{14}\xtic{15}\xtic{16}\xtic{17}\xtic{18}\xtic{19}\xtic{20}\xtic{21}\xtic{22}; 
\draw [thin]\ytic{1}\ytic{2}\ytic{3}\ytic{4}\ytic{5}\ytic{6}\ytic{7}\ytic{8}\ytic{9};
\fill [pattern=north west lines, pattern color=blue] (3,0) 
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,-5)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0) --(3,0);
\fill [fill=lightgray] (8,0) 
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,1) -- ++(1,0)
-- ++(0,-2)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0)
-- ++(0,-1)-- ++(-1,0) --(8,0);
\draw [thick] 
(0,1) -- ++(1,0) -- 
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,-2) -- ++(1,0) -- % update #1
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,-4)-- ++(1,0) -- %update #2
++(0,-1)-- ++(1,0) -- %update #3
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0) --
++(0,-4) -- ++(1,0) -- %update #3
++(0,1) -- ++(1,0) --
++(0,1) -- ++(1,0);
\draw (2,0) node [below] {$n_1$};
\draw [->] (5,0) -- ++(0,-1) node [below] {$n'_1$};
\draw (7,0) node [below] {$n_2$}; 
\draw (9,0) node [below] {$n_3$};
\draw [->] (12,0) -- ++(0,-1) node [below] {$n'_2$};
\draw [->] (13,0) -- ++(0,-1) node [below] {$n'_3$};
\draw  [|<->|] (0,-3.5) to node [below] {$Y_1$} ++(3,0);
\draw  [|<->|] (3,-3.5) to node [below] {$T_1$} ++(2,0);
\draw  [|<->|] (3,-5.5) to node [below] {$Y_2$} ++(5,0);
\draw  [|<->|] (8,-5.5) to node [below] {$T_2$} ++(4,0);
\draw  [|<->|] (8,-3.5) to node [below] {$Y_3$} ++(2,0);
\draw  [|<->|] (10,-3.5) to node [below] {$T_3$} ++(3,0);
\draw[<-] (12.5,3.5) to [out=110,in=250] ++(1,4) node [above] {$Q_3$};
\draw[<-] (7.5,3.5) to [out=110,in=250] ++(1,4) node [above] {$Q_2$};
\end{tikzpicture}
\caption{The age process $A_m(n)$ at the monitor when updates from the source pass through a queue. %(The system is initialized with a fresh arrival prior to slot $0$.
}
\label{fig:DTqueue}
\end{figure}

==> Privacy Leakage/macros.tex <==
\newcommand{\RED}[1]{{\color{red}{#1}}}
\DeclareMathOperator{\Cv}{Cv}

%\newcommand{\nn}{\nonumber\\}
\long\def\/*#1*/{}



\newcommand{\Ie}{\textit{i.e., }}





\renewcommand{\P}{\mathbb{P}}
\renewcommand{\L}{\mathcal{L}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\mcN}{\mathcal{N}}
\newcommand{\n}{\mathbf{n}}

\usepackage[normalem]{ulem}
\newcommand\redout{\bgroup\markoverwith{\textcolor{red}{\rule[.5ex]{2pt}{0.4pt}}}\ULon}
\newcommand{\edit}[2]{\redout{#1}{~\textcolor{blue}{#2}}}

\newcommand{\cn}{\textcolor{red}{[\raisebox{-0.2ex}{\tiny\shortstack{citation\\[-1ex]needed}}]}}

% Editing macros

\newcommand{\todo}[1]{\textcolor{red} {\textbf{Todo: #1}}}
\newcommand{\ads}[1]{\textcolor{purple}{\textbf{ADS:} #1}}
\newcommand{\rdy}[1]{\textcolor{blue}{\textbf{RDY:} #1}}
\newcommand{\nm}[1]{\textcolor{orange}{\textbf{NM:} #1}}
\newcommand{\ns}[1]{\textcolor{teal}{\textbf{NS:} #1}}



%\newcommand{\cn}{\textcolor{red}{[\raisebox{-0.2ex}{\tiny\shortstack{citation\\[-1ex]needed}}]}}

 
% \newcommand{\eqnlabel}[1]{\label{eqn:#1}}
% \newcommand{\eqnref}[1]{(\ref{eqn:#1})}

%\newtheorem{claim}{Claim}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
